Lambda-Policy Iteration with Randomization for Contractive Models with Infinite Policies: Well-Posedness and Convergence (Extended Version)

Abstract dynamic programming models are used to analyze $\lambda$-policy iteration with randomization algorithms. Particularly, contractive models with infinite policies are considered and it is shown that well-posedness of the $\lambda$-operator plays a central role in the algorithm. The operator is known to be well-posed for problems with finite states, but our analysis shows that it is also well-defined for the contractive models with infinite states studied. Similarly, the algorithm we analyze is known to converge for problems with finite policies, but we identify the conditions required to guarantee convergence with probability one when the policy space is infinite regardless of the number of states. Guided by the analysis, we exemplify a data-driven approximated implementation of the algorithm for estimation of optimal costs of constrained linear and nonlinear control problems. Numerical results indicate potentials of this method in practice.

==> recycle.tex <==
\begin{algorithm2e}
\caption{Data-driven $\lambda$-PIR}
\label{alg:lpi}
\DontPrintSemicolon
%\LinesNumbered
\KwIn{probelm data $\mathbf{D}$, algorithm data $\mathbf{A}$, initial parameter $\theta_0$, sample size $S$}
\KwOut{$\theta$, the trained parameter}
$\theta\leftarrow \theta_0$\;
\For{$k\leftarrow 1$ \KwTo $K$}{
Initialize $\mathbf{x}\in\mathbb{R}^{n\times S}$, $\mathbf{v}\in\mathbb{R}^{S}$\;
\For{$s\leftarrow 1$ \KwTo $S$}{
$x_0\sim\mathcal{X}_0$, $b\sim\text{Ber}(p_k)$\;
\uIf{$b==1$}{$v\leftarrow \inf_{u\in U(x_0)}g(x_0,u)+\gamma \Tilde{J}(f(x_0,u),\theta)$}
\Else{$L\sim\text{Ge}(\lambda)$, $v=0$, Initialize $\mathbf{t}\in\mathbb{R}^{n\times L}$, $\mathbf{u}\in\mathbb{R}^{L}$, $\mathbf{t}_1\leftarrow x_0$\;
\For{$\ell \leftarrow 1$ \KwTo $L$}{
$\mathbf{u}_{\ell}\in\argmin_{u\in U(\mathbf{t}_{\ell})}g(\mathbf{t}_{\ell},u)+\gamma \Tilde{J}(f(\mathbf{t}_{\ell},u),\theta)$, $v\leftarrow v+\gamma^{\ell-1}g(\mathbf{t}_{\ell},\mathbf{u}_{\ell})$
}
$v\leftarrow v+\gamma^{L}\Tilde{J}(f(\mathbf{t}_{L},\mathbf{u}_{L}),\theta)$
}
$\mathbf{x}_s=x_0$, $\mathbf{v}_s=v$
}
$\theta\in \argmin_{\theta\in\Theta}\sum_{s\in S}|\Tilde{J}(\mathbf{x}_s,\theta)-\mathbf{v}_s|^2$
}
\end{algorithm2e}



\usepackage{graphicx}
\usepackage{subfig}

\begin{figure}[h]
  \centering
  \subfloat[System behavior with different cost function estimate, $0$ stands for untrained and numbers for training iterations.]{\includegraphics[width=0.51\textwidth]{l4dc/train.pdf}\label{fig:f1}}
  \hfill
  \subfloat[System behavior with trained and untrained cost function from different initial states.]{\includegraphics[width=0.49\textwidth]{l4dc/initial.pdf}\label{fig:f2}}
  \caption{Closed-loop system behavior under ADP control.}
  \label{fig:f}
\end{figure}


The following result shows that the operator $T^{(\lambda)}_\mu$ defined point-wise is no difference compared one defined by convergence in norm.
\begin{theorem}\label{thm:53}
	Consider sequence $\{T^{(\lambda_n)}_\mu J\}$ defined by $T^{(\lambda_n)}_\mu J=(1-\lambda)\sum_{\ell=1}^n  \lambda^{\ell-1}T_\mu^{\ell}J$. The sequence $\{T^{(\lambda_n)}_\mu J\}$ converges to some element $T^{(\lambda_\infty)}_\mu J\in\mathcal{B}(X)$. In addition, it coincides with the function $T^{(\lambda)}_\mu J$ defined by point-wise limit, viz., $T^{(\lambda_\infty)}_\mu J=T^{(\lambda)}_\mu J$.
\end{theorem}
Note that the above result does not stand for the more general operator $T^{(w)}_\mu$, when $X$ has infinite cardinality. The counterexample is given in the extended version of this paper \cite{li2019abstract}.

On the other hand, the monotonicity property of $T^{(w)}_\mu$ and $T^{(\lambda)}_\mu$ can be easily followed from the monotonicity property of $T_\mu$. This is summarized in the following theorem. The proof is neglected.
\begin{theorem}\label{thm:3}
	Let the set of mappings $T_\mu:\mathcal{B}(X)\to \mathcal{B}(X)$, $\mu\in\mathcal{M}$ satisfy Assumptions~\ref{asm:contra} and \ref{asm:mon}. Then the mappings $T_\mu^{(w)}:\mathcal{B}(X)\to\mathcal{B}(X)$ defined in Eq.~\eqref{eq:thm1def} is monotonic in the sense that 
	\begin{equation*}
    J\leq J'\implies T_\mu^{(w)}J\leq T_\mu^{(w)}J',\;\forall x\in X,\,\mu\in \mathcal{M}.
\end{equation*}
\end{theorem}
